Benchmarking Quality-Diversity Algorithms on Neuroevolution for Reinforcement Learning

We present a Quality-Diversity benchmark suite for Deep Neuroevolution in Reinforcement Learning domains for robot control. The suite includes the definition of tasks, environments, behavioral descriptors, and fitness. We specify different benchmarks based on the complexity of both the task and the agent controlled by a deep neural network. The benchmark uses standard Quality-Diversity metrics, including coverage, QD-score, maximum fitness, and an archive profile metric to quantify the relation between coverage and fitness. We also present how to quantify the robustness of the solutions with respect to environmental stochasticity by introducing corrected versions of the same metrics. We believe that our benchmark is a valuable tool for the community to compare and improve their findings. The source code is available online: https://github.com/adaptive-intelligent-robotics/QDax

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> old_files/2_prelim.tex <==
% \section{Preliminaries}

% RL domains are formulated as a Markov Decision Process (MDP) \cite{sutton2018reinforcement} described by the tuple $(\mathcal{S}, \mathcal{A}, r, \gamma, T)$. The initial state $\vec{s_0}$ is first sampled from a initial state distribution. At each following timestep $t$, an action $\vec{a_t}$ is then taken in state $\vec{s_t}$ by a policy $\pi_{\vec{\theta}}(\vec{a_t}|\vec{s_t})$ with parameters $\vec{\theta}$ resulting in the next state $\vec{s_{t+1}}$. 
% In the context of deep neuroevolution, the policy is represented as a neural network with its parameters, $\vec{\theta}$. 
% The episode is rolled out a fixed number of timesteps, $T$ resulting in a trajectory of states $\tau=(\vec{s_0},\vec{s_1},...,\vec{s_T})$.

% In QD, both the fitness $f$ and behavioural descriptor $bd$ are defined as functions of the state trajectory $\tau$.
% % \begin{align*}
% %     Fit &= f_{fit}(\tau) = R(\tau) \\
% %     BD &= f_{bd}(\tau)
% % \end{align*}
% %Fitness is defined as a function of the state trajectory and is not limited to be the sum of discounted rewards as in the conventional RL formulation. 
% In this paper, a task consists of the fitness and behavioural descriptor definitions along with a defined MDP usually given by the environment. This formulation has also been used and explored in recent works at the intersection of QD and RL~\cite{colas2020scaling, nilsson2021policy, tjanaka2022approximating}.




==> old_files/3_methods.tex <==
% \section{Methods}

% \subsection{High-dimensional search-space}
% Traditional GAs can have issues with high-dimensional search spaces. Such et al [Genetic Algorithms Are a Competitive Alternative for Training Deep Neural Networks for Reinforcement Learning] have shown that even the best GAs are not able to find solutions for a continuous control task. Colas et al. [Scaling MAP-Elites to Deep Neuroevolution] have shown that you can scale Quality-Diversity to larger search spaces with their algorithm ME-ES.  

% \begin{itemize}
%     \item Neural Networks seem to be a good example of high-dimensional search spaces
%     \item NN Controllers for Gym Tasks could be an interesting task to check how well the algorithm is able to find solutions in a high dimensional search space
%     \item We could reuse the tasks that we have in other sections and simply use a large NN to check how well we can do neuro-evolution
% \end{itemize}

% \begin{itemize}
%     \item HTE, HBR: The search space can be decomposed hierarchically to find better solutions (e.g. chaining different controllers) in a reduced search space
%     \item PGA-ME: Use gradient descent to guide the solutions 
%     \item ME-ES
% \end{itemize}


% \subsection{Uncertainty and stochasticity QD algorithms}

% QD algorithms rely on estimating the quality --fitness-- and characterising the behaviour --BD-- induce by a solution. In most QD algorithms this estimation is done based on a unique evaluation of the considered solution in the environment.  
% However, in most environments two evaluations of the exact same solution might lead to different fitness and BD estimations \cite{}. This lack of reproducibility can arise from stochasticity in the dynamic of the environments, or in the measurements done in this environment to compute the fitness and BD, or alternatively to slight change in the initialisation of the environment. 
% Thus, this problem raises two main questions:
% \begin{itemize}
%     \item How to estimate the true fitness and BD of a given solution while staying sample-efficient?
%     \item How to enforce solutions that are more reproducible?
% \end{itemize}
% Most current QD algorithms do not have mechanisms to tackle these problems, and the simple approach when this limitation becomes too important has been to augment the traditional MAP-Elites loop with some additional sampling of each solution to try to get a better estimate of the fitness and BD of solutions \cite{}. 
% However, recently some other works have proposed explicit mechanisms to tackle this issue \cite{}.
% To study the performance of such approaches we propose below a set of tasks with different types of stochasticity or uncertainty.

% %\subsubsection{Improving fitness and BD approximation in stochastic environments}
% \subsubsection{Robustness of repertoires}
% We propose a first set of tasks which focus on the first limitation that arise in stochastic environment: estimating the true fitness and BD of a solution.
% In an effort to try to de-correlate the two problems, we consider tasks and controllers for which all solutions are equally reproducible. Thus, we only consider open-loop control tasks.

% \paragraph{Tasks}
% The first set of tasks consist in usual QD tasks with additional Gaussian noise on the fitness and BD of each solution.
% \begin{itemize}
%     \item Simulated 8-degrees-of-freedom arm control, with Gaussian fitness and BD noise
%     \item Simulated hexapod robot control, with Gaussian fitness and BD noise
% \end{itemize}

% \paragraph{Analysis}
% The outcome of algorithms on these tasks can be analysed using the reveal archive filled using the ground truth values of fitness and BD for each solution. 


% %\subsubsection{Enforcing reproducible solutions in stochastic environments}
% \subsubsection{Robustness of solutions in niches of repertoire}
% We propose two level of tasks to study the reproducibility of solutions generated by a QD algorithm. 

% \paragraph{Tasks}
% The first level consist of hand-design tasks for which reproducible and non-reproducible solutions are easily differentiable. 
% \begin{itemize}
%     \item Simulated 8-degrees-of-freedom arm control, with Gaussian noise in the last actuator of the arm
% \end{itemize}

% \paragraph{Analysis}
% These tasks allow to easily distinguish reproducible and non-reproducible solutions. Thus, the outcome of algorithms can be compared using the distribution of all final solutions reproducibility.

% \paragraph{Tasks}
% The second level consist of closed-loop controlled tasks with stochastic initialisation
% \begin{itemize}
%     \item Simulated hexapod robot control, with closed-loop control and random joint initialisation
% \end{itemize}

% \paragraph{Analysis}
% The outcome of algorithms on these tasks can be analysed using the reveal archive filled using approximation of the ground truth values of fitness and BD of each solution based on 50 reevaluations of the same solution in the environment. 




% % \subsection{Dimension 4: Efficiency}
% % Efficiently illuminate the BD space (evaluated via QD-score and coverage).

% % Depends on the application - 
% % Possible Metrics:
% % \begin{itemize}
% %     \item Number of evaluations: important in applications where evaluations are very expensive (i.e. real world - cannot be sped up by simulation/hardware acceleration) or evaluations are dangerous/unsafe.
% %     \item Runtime (Wall Clock Time): important in applications where fast simulation. Given no additional overhead (i.e. training additional models, evaluating surrogate models, etc.), less evaluations would also usually translate into lower wall clock time.
% % \end{itemize}

% % \subsubsection{Optimization Strategies}
% % Conventionally, QD algorithms rely on mutation based operators derived from Genetic Algorithms (GAs) to perturb parameters during search. However, while having the advantage of being a black-box optimizer and being effective for exploration, this strategy typically requires many evaluations. More efficient optimization methods that leverage gradients can also be used in QD. Gradients of the objective function~\cite{} and even diversity gradient~\cite{}.

% % \subsubsection{Model-Based QD}
% % A line of work that attempts to address sample-efficiency, now referred to as \textit{model-based quality-diversity} methods, is through the use of models. Model-based QD methods are particularly useful where number of evaluations is considered as the metric as it aims to directly reduce this.
% % Surrogate-Assisted Illumination (SAIL) \cite{gaier2018data} first introduced the use of surrogate models for QD algorithms. SAIL integrates surrogate models, in the form of Gaussian Process (GP) models, to approximate the objective function and reduce the number of evaluations for the computationally expensive application of aerodynamic design. Another algorithm called M-QD \cite{keller2020model} later follows up on this idea and used neural network models that map the parameter space to the behaviour and fitness space as a surrogate model. They demonstrate this on robotic pushing and placing tasks. Dynamics-Aware Quality-Diversity (DA-QD) \cite{lim2021dynamics} is another approach which instead uses learnt dynamics models as a surrogate model. DA-QD introduced the concept of the imagined repertoire which allows QD to be performed fully in imagination using the learnt dynamics models. The dynamics models are trained incrementally and online as data is collected through evaluations. DA-QD showed a significant ($\approx$20 time) increase in sample-efficiency.

% % \subsubsection{Hardware Acceleration}

% When the number of evaluations are not important, hardware acceleration can be used to massively parallels evaluations. This can speed up the QD algorithms in terms of wall-clock time.

==> old_files/old_abstract.tex <==

%Quality-Diversity (QD) algorithms have recently become a commonly used tool across a wide range of applications.
%This increase in usage and popularity has resulted in many advances within this field, especially when used in neuroevolution for reinforcement learning tasks.
%However, with progress in QD algorithms continuing at this pace, a lack of standardized benchmarks and metrics makes it difficult to rigorously compare new algorithmic innovations effectively within this field.
%This paper proposes a set of two benchmark QD tasks across six environments of varying levels of difficulty aimed at evaluating QD algorithms for neuroevolution in reinforcement learning domains.
%We also identify key challenges in this domain and set about evaluation procedures and metrics to best evaluate QD algorithms in this setting.

==> old_files/old_body.tex <==

% % \section{Dimension 1: Derailment}

% % The \textit{Derailment} was introduced in First Return then Explore [??].
% % %
% % It refers to the difficulty encountered by exploratory algorithms when trying to reach a previously visited state.
% % %
% % For example, applying a normal mutation to the parameters of a Deep Neural Network policy does not guarantee the agent to reach a nearby final state.

% % That problem is very common in Robotic Manipulation tasks.
% % %
% % For example, Go-Explore has been applied to a robotic grasping task, where a Fetch robot is required to explore its environment to pick up an object and place it in one of its shelves.
% % %
% % Another similar problem, similar to problems handled via IMGEPs, consists of an arm with a gripper, that can move to grab sticks, that can be used to manipulate objects.

% % The problem of derailment also appears in Robotic Locomotion tasks.
% % %
% % For example, in the Humanoid Locomotion task, a small change in the policy may lead to some instability that can make the agent fall.
% % %
% % In such case, a small perturbation of parameters may lead to completely different final states.

% % \begin{itemize}
% %     \item Robotic Grasping Task (First Return then Explore):
% %     \begin{itemize}
% %         \item \textit{Genotype:} 2 Fully connected layers + layers of gated recurrent units. (one network for actor, the other for critic).
% %         \item \textit{Fitness:} None ?
% %         \item \textit{BD:} Room Number, Level Number, Number of keys, (x, y) position
    
% %     \end{itemize}

% %     \item Robotic Grasping Task (Lorenzo):
% %     \begin{itemize}
% %         \item \textit{Genotype:} All joints successive targets
% %         \item \textit{Fitness:} None
% %         \item \textit{BD:} 1 value to identify the object, X and Y coordinates of the end position of that object (15 objects).
% %     \end{itemize}

% %     \item Robotic Locomotion Task (Humanoid):
% %         \begin{itemize}
% %             \item \textit{Genotype:} MLP with two hidden layers of size 64 [??] or of size 256 [??]
% %             \item \textit{Fitness:} a mixture of velocity along the $x$-axis and costs for joint torques. [??]
% %             \item \textit{BD:} final $x,y$ position. [??]
% %         \end{itemize}
% % \end{itemize}

% % \textbf{My humble opinion:} I do not think the derailment should be a main direction to define benchmarking environments. 
% % %
% % However, if we want to focus on Robotic Locomotion tasks, the derailment seems like a good justification of the difficulty to solve some environments such as the Humanoid. 

% % Possible metrics to characterise derailment of a task:
% % \begin{itemize}
% %     \item \textbf{Evolvability of solutions}.
% % \end{itemize}

% \section{Dimension 2: Uncertain environment and reproducibility of solutions}

% QD algorithms rely on estimating the quality --fitness-- and characterising the behaviour --BD-- induce by a solution. In most QD algorithms this estimation is done based on a unique evaluation of the considered solution in the environment.  
% However, in most environments two evaluations of the exact same solution might lead to different fitness and BD estimations \cite{}. This lack of reproducibility can arise from stochasticity in the dynamic of the environments, or in the measurements done in this environment to compute the fitness and BD, or alternatively to slight change in the initialisation of the environment. 
% Thus, this problem raises two main questions:
% \begin{itemize}
%     \item How to estimate the true fitness and BD of a given solution while staying sample-efficient?
%     \item How to enforce solutions that are more reproducible?
% \end{itemize}
% Most current QD algorithms do not have mechanisms to tackle these problems, and the simple approach when this limitation becomes too important has been to augment the traditional MAP-Elites loop with some additional sampling of each solution to try to get a better estimate of the fitness and BD of solutions \cite{}. 
% However, recently some other works have proposed explicit mechanisms to tackle this issue \cite{}.
% To study the performance of such approaches we propose below a set of tasks with different types of stochasticity or uncertainty.

% \subsection{Improving fitness and BD approximation in stochastic environments}

% We propose a first set of tasks which focus on the first limitation that arise in stochastic environment: estimating the true fitness and BD of a solution.
% In an effort to try to de-correlate the two problems, we consider tasks and controllers for which all solutions are equally reproducible. Thus, we only consider open-loop control tasks.

% \subsubsection{Tasks}
% The first set of tasks consist in usual QD tasks with additional Gaussian noise on the fitness and BD of each solution.
% \begin{itemize}
%     \item Simulated 8-degrees-of-freedom arm control, with Gaussian fitness and BD noise
%     \item Simulated hexapod robot control, with Gaussian fitness and BD noise
% \end{itemize}

% \subsubsection{Analysis}
% The outcome of algorithms on these tasks can be analysed using the reveal archive filled using the ground truth values of fitness and BD for each solution. 


% \subsection{Enforcing reproducible solutions in stochastic environments}

% We propose two level of tasks to study the reproducibility of solutions generated by a QD algorithm. 

% \subsubsection{Tasks}
% The first level consist of hand-design tasks for which reproducible and non-reproducible solutions are easily differentiable. 
% \begin{itemize}
%     \item Simulated 8-degrees-of-freedom arm control, with Gaussian noise in the last actuator of the arm
% \end{itemize}

% \subsubsection{Analysis}
% These tasks allow to easily distinguish reproducible and non-reproducible solutions. Thus, the outcome of algorithms can be compared using the distribution of all final solutions reproducibility.

% \subsubsection{Tasks}
% The second level consist of closed-loop controlled tasks with stochastic initialisation
% \begin{itemize}
%     \item Simulated hexapod robot control, with closed-loop control and random joint initialisation
% \end{itemize}

% \subsubsection{Analysis}
% The outcome of algorithms on these tasks can be analysed using the reveal archive filled using approximation of the ground truth values of fitness and BD of each solution based on 50 reevaluations of the same solution in the environment. 

% \section{Dimension 3: High-dimensional search-space}

% Traditional GAs can have issues with high-dimensional search spaces. Such et al [Genetic Algorithms Are a Competitive Alternative for Training Deep Neural Networks for Reinforcement Learning] have shown that even the best GAs are not able to find solutions for a continuous control task. Colas et al. [Scaling MAP-Elites to Deep Neuroevolution] have shown that you can scale Quality-Diversity to larger search spaces with their algorithm ME-ES.  

% \begin{itemize}
%     \item Neural Networks seem to be a good example of high-dimensional search spaces
%     \item NN Controllers for Gym Tasks could be an interesting task to check how well the algorithm is able to find solutions in a high dimensional search space
%     \item We could reuse the tasks that we have in other sections and simply use a large NN to check how well we can do neuro-evolution
% \end{itemize}

% \begin{itemize}
%     \item HTE, HBR: The search space can be decomposed hierarchically to find better solutions (e.g. chaining different controllers) in a reduced search space
%     \item PGA-ME: Use gradient descent to guide the solutions 
%     \item ME-ES
% \end{itemize}


% \section{Dimension 4: Efficiency}
% Efficiently illuminate the BD space (evaluated via QD-score and coverage).

% Depends on the application - 
% Possible Metrics:
% \begin{itemize}
%     \item Number of evaluations: important in applications where evaluations are very expensive (i.e. real world - cannot be sped up by simulation/hardware acceleration) or evaluations are dangerous/unsafe.
%     \item Runtime (Wall Clock Time): important in applications where fast simulation. Given no additional overhead (i.e. training additional models, evaluating surrogate models, etc.), less evaluations would also usually translate into lower wall clock time.
% \end{itemize}

% \subsection{Optimization Strategies}
% Conventionally, QD algorithms rely on mutation based operators derived from Genetic Algorithms (GAs) to perturb parameters during search. However, while having the advantage of being a black-box optimizer and being effective for exploration, this strategy typically requires many evaluations. More efficient optimization methods that leverage gradients can also be used in QD. Gradients of the objective function~\cite{} and even diversity gradient~\cite{}.

% \subsection{Model-Based QD}
% A line of work that attempts to address sample-efficiency, now referred to as \textit{model-based quality-diversity} methods, is through the use of models. Model-based QD methods are particularly useful where number of evaluations is considered as the metric as it aims to directly reduce this.
% Surrogate-Assisted Illumination (SAIL) \cite{gaier2018data} first introduced the use of surrogate models for QD algorithms. SAIL integrates surrogate models, in the form of Gaussian Process (GP) models, to approximate the objective function and reduce the number of evaluations for the computationally expensive application of aerodynamic design. Another algorithm called M-QD \cite{keller2020model} later follows up on this idea and used neural network models that map the parameter space to the behaviour and fitness space as a surrogate model. They demonstrate this on robotic pushing and placing tasks. Dynamics-Aware Quality-Diversity (DA-QD) \cite{lim2021dynamics} is another approach which instead uses learnt dynamics models as a surrogate model. DA-QD introduced the concept of the imagined repertoire which allows QD to be performed fully in imagination using the learnt dynamics models. The dynamics models are trained incrementally and online as data is collected through evaluations. DA-QD showed a significant ($\approx$20 time) increase in sample-efficiency.

% \subsection{Hardware Acceleration}
% When the number of evaluations are not important, hardware acceleration can be used to massively parallels evaluations. This can speed up the QD algorithms in terms of wall-clock time.


% \section{Dimension 5: High-dimensional BD space}

% High-Dimensional BD spaces reduce the evolutionary selection pressure. It is therefore important for the QD algorithm to be able to have selection mechanisms that can overcome large dimensional BD spaces. Furthermore, a large BD space means that the number of solutions will exponentially grow and cannot easily be stored if the number grows too quickly. 

% \begin{itemize}
%     \item Compare Projected QD scores along a certain dimension of interest in the BD space. 
%     \item Compare X,Y locomotion for hexapods with 2D and 8D archives (where the 6 additional dimensions can be the duty cycle)
%     \item Downstream tasks, e.g. MCTS in 8-Dimensional RTE vs 2-Dimensional RTE 
% \end{itemize}

% \begin{itemize}
%     \item HTE : Reusing Behaviours from lower levels to avoid exponential growth. Push for exploration along different dimensions on different layers instead of using a single layer.
%     \item AURORA & RUDA: Automatic Encoding of large BD dimensions toward a small space
% \end{itemize}

% \newpage
% \section{Copy Deep-grid paper}

% \subsection{Simulated 8-degrees-of-freedom arm control} 

% Inspired by \cite{}, this task aim to find how to access all the points reachable by a simulated 8-Degree-of-Freedom (8-DoF) arm, while minimising the variance between the different angles applied in each of its DoF.
% \begin{itemize}
%     \item[--] \emph{Controller:} set of 8 real-valued angles: $\vec{\theta}=(\theta_i)_{1<i<8}$.
%     \item[--] \emph{Descriptor:} $(x_{hand},y_{hand})$ position of the end-effector.
%     \item[--] \emph{Fitness:} variance of the angles $(\theta_i)_{1<i<8}$:
%     $$f(\vec{\theta})=-V((\theta_i)_{1<i<8}) = -\frac{1}{8}\sum_{i=1}^{8}{(\theta_i-\overline{\theta})^2}$$
%     \item[--] \emph{Physics simulator:} none.
% \end{itemize}

% \subsection{Simulated hexapod robot control} the aim of this task taken from \cite{} is to learn how to walk in every direction following circular trajectories with a simulated hexapod robot with 3-DoF per leg.
% \begin{itemize}
%     \item[--] \emph{Controller:} set of periodic functions, applied in each DoF of the robot and characterised by their amplitude, phase, and duty cycle: $\vec{x}=(A_i, \phi_i, \gamma_i)_{i=[1,18]}$. 
%     \item[--] \emph{Descriptor:} $(x_{hexapod},y_{hexapod})$ robot final position.
%     \item[--] \emph{Fitness:} angle difference between the final orientation of the robot $\alpha(\vec{x})$ and the tangent of the circle through its start and end position $\beta(\vec{x})$: 
% \begin{center} $f(\vec{x})=-| \alpha(\vec{x}) - \beta(\vec{x}) | $ \end{center}
%     \item[--] \emph{Physics simulator:} Dart \cite{}, using RobotDart library \cite{}.
% \end{itemize}

% \subsection{Simulated lunar lander task} this task aims to land a lunar lander on a planet, controlling its 4 propellers. It is directly inspired by the Gym Lunar-lander task \cite{}. 
% \begin{itemize}
%     \item[--] \emph{Controller:} Each propeller $i$ follows $P_i = A_i * t + B_i$, where $\vec{C}=(A_i, B_i)_{1<i<4}$ are real-valued coefficients.
%     \item[--] \emph{Descriptor:} $(x_{lander},\theta_{lander})$ final position along x and orientation of the lander.
%     \item[--] \emph{Fitness:} sum of the normalised final velocity and total time taken to land: $f(\vec{C})=-(v_{norm} + \dot{\theta}_{norm} + t_{norm})$
%     \item[--] \emph{Physics simulator:} Box2D \cite{}, using Robox2D library \cite{}.
% \end{itemize}

% \subsection{Simulated air arm task} this task aim to find how to access all the points reachable by a simulated 4-DoF arm, minimising the energy.
% \begin{itemize}
%     \item[--] \emph{Controller:} each joint $i$ follows the position command $\theta_i = A_i * t + B_i$, where $\vec{C}=(A_i, B_i)_{1<i<4}$ are real-valued coefficients.
%     \item[--] \emph{Descriptor:} $(x_{hand},y_{hand})$ position of the end-effector.
%     \item[--] \emph{Fitness:} sum over time of the actuators speed squared: $$f(\vec{\theta})=-\sum_{t=0}^T\sum_{i=1}^4(\dot{\theta}_t^i)^2$$
%     \item[--] \emph{Physics simulator:} Box2D \cite{}, using Robox2D library \cite{}.
% \end{itemize}

% \subsection{Simulated air hockey task} Inspired by \cite{}, this task aim to find how to reach all the points of a square with a puck launched by a simulated 4-DoF arm, minimising the energy.
% \begin{itemize}
%     \item[--] \emph{Controller:} set of 8 real-valued joint positions, corresponding to the 4 initial and 4 final positions of each of the 4 joints: $\vec{\theta}=(\theta_0^i, \theta_T^i)_{1<i<4}$.
%     \item[--] \emph{Descriptor:} $(x_{puck},y_{puck})$ final position of the puck.
%     \item[--] \emph{Fitness:} same as the simulated air arm task.
%     \item[--] \emph{Physics simulator:} Box2D \cite{}, using Robox2D library \cite{}.
% \end{itemize}

% \subsection{Simulated hexapod robot control} 
% \begin{itemize}
%     \item[--] \emph{Controller:} NN which takes as input the current state of the hexapod (joint position, joint velocity, robot position and current timestep) and outputs the next-step target joint position: $(\theta_i)_{1<i<18}$. 
% \end{itemize}

% \subsection{Simulated lunar lander task} 
% \begin{itemize}
%     \item[--] \emph{Controller:} NN which takes as input the current state of the lander (lander linear and rotational position and velocity, timestep) and outputs the next-step 4 propeller command: $(P_i)_{1<i<4}$.
% \end{itemize}

% \subsection{Simulated air arm task} 
% \begin{itemize}
%     \item[--] \emph{Controller:} NN which takes as input the current state of the arm (joint position and velocity, timestep) and outputs the next-step 4 joint positions: $(\theta_i)_{1<i<4}$.
% \end{itemize}

% \subsection{Simulated air hockey task} 
% \begin{itemize}
%     \item[--] \emph{Controller:} NN which takes as input the current state of the arm (joint position and velocity, timestep) and outputs the next-step 4 joint positions: $(\theta_i)_{1<i<4}$.
% \end{itemize}

% \input{tables/tasks}

==> old_files/old_metrics.tex <==

% \section{Metrics}

% \subsection{Studying the Evolution of the Quality and Diversity of the Container}

% \begin{enumerate}
%     \item Compare the speed of different algorithms.
%     \item See if the algorithms have converged.
% \end{enumerate}


% \subsubsection{Coverage}

% The coverage metric estimates the percentage the BD space filled by the container.
% %
% To calculate it, the (bounded) BD space is discretised into a grid, and the coverage corresponds to the percentage of grid cells containing at least one individual from the container.

% \subsubsection{QD Score}

% The QD Score estimates the overall performance and coverage of the container.
% %
% Before computing it, all the QD scores from all individuals are normalised between 0 and 1.
% %
% Then, as for the Coverage metric, the containers are projected onto a BD space grid; in each cell only the best performing individual is kept.
% %
% The QD score then corresponds to the sum of all fitness scores in the grid.



% \subsubsection{Max Fitness}

% The maximum fitness of a container is the highest achieved fitness among all individuals present in the container.


% \subsection{Evaluating the Quality and Diversity of Returned Containers}

% Can be useful for studying the properties of containers returned by a QD algorithm after a finite number of evaluations/iterations.

% \subsubsection{Coverage per Minimum Performance} 

% \label{sec:cov_per_min_fit}

% The containers returned by any QD algorithm always result in a trade-off between the diversity and the total performance of the solutions from the container.
% %
% To evaluate the coverage depending on the quality of the solutions, we study the evolution of the coverage given several minimum performance scores.
% %
% With a performance $f_{min}$ and a BD space discretised into a grid, we define the \textit{"coverage given minimum performance $f_{min}$"} as: the number of cells filled with policies whose performance is higher than $f_{min}$.

% The coverage is calculated by discretising the Behavioural Descriptor (BD) space into a grid.
% %
% The coverage then corresponds the number of grid cells containing at least one policy from the container.

% \begin{figure*}[t]
%     \centering
%     \includegraphics{figures/02_iclr_coverage_per_fitness.pdf}
%     \caption{Coverage per Minimum Fitness}.
%     \label{fig:my_label_1}
% \end{figure*}

% \subsubsection{Coverage per Grid Resolution}

% We define the \textit{"coverage given grid resolution $r$"} as: the number of cells filled after having projected the container in a grid where each axis is uniformly split into $r$ portions.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.3\textwidth]{figures/coverage_per_grid_resolution.png}
%     \caption{Coverage per Grid Resolution}.
%     \label{fig:my_label_2}
% \end{figure*}

% \subsubsection{Particle-based Entropy ?}

% Kind of equivalent to average novelty score. Can be useful in unbounded BD spaces or BD spaces that are not easily discretisable.

% Drawback: Difficult to compare algorithms with different numbers of individuals.

% \subsection{Computational Complexity}

% All QD algorithms and implementations do not provide the same computational efficiency and time complexity.
% %
% To take into account those characteristics, we propose to study the evolution of the \textit{total wall time} for each variant.
% %
% The wall time is defined as the amount of time spent since the algorithm has started.
% %
% Then by comparing the total wall time for each algorithm, we can derive the difference in terms of computational overhead (i.e. the time that is not spent to evaluate individuals).
% %

% % \begin{itemize}
% %     \item reporting how quickly we generate some results can be useful.
% %     \item studying computational overhead
% % \end{itemize}




% \subsection{Genotype size}
% To investigate the effect of the number of parameters on the different algorithms, we propose using neural networks of different size to evaluate the effect of the number of parameters on QD algorithms. Issue with this is that it might be prone to lottery ticket phenomena and we might not actually evaluate the ability of QD algorithms to optimise large number of parameters? 



% \begin{equation}
%     Robustness = f(\theta_i)_{elite} - \mu_f^{N}(\theta_i)
% \end{equation}
